Towards Effective Collaborative Learning in Long-Tailed Recognition

Real-world data usually suffers from severe class imbalance and long-tailed distributions, where minority classes are significantly underrepresented compared to the majority ones. Recent research prefers to utilize multi-expert architectures to mitigate the model uncertainty on the minority, where collaborative learning is employed to aggregate the knowledge of experts, i.e., online distillation. In this paper, we observe that the knowledge transfer between experts is imbalanced in terms of class distribution, which results in limited performance improvement of the minority classes. To address it, we propose a re-weighted distillation loss by comparing two classifiers' predictions, which are supervised by online distillation and label annotations, respectively. We also emphasize that feature-level distillation will significantly improve model performance and increase feature robustness. Finally, we propose an Effective Collaborative Learning (ECL) framework that integrates a contrastive proxy task branch to further improve feature quality. Quantitative and qualitative experiments on four standard datasets demonstrate that ECL achieves state-of-the-art performance and the detailed ablation studies manifest the effectiveness of each component in ECL.

==> Figures/Texs/fig_tau.tex <==
\begin{figure}[t!]
	\centering
	\flushleft
	\begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=1\linewidth,grid=False]{Figures/Tau_BC_loss.pdf}
    \end{overpic}
	\caption{todo xxx}
	% \vspace{-10pt}
	\label{fig:tau}
\end{figure}

==> Tables/Result_new_baseline.tex <==
\begin{table}[t!]
\centering
\caption{Results of reproduced methods based on our CE++ on CIFAR-100-LT ($\gamma=100$). Each method gets improved to some extent compared to the original results in Tab.~\ref{Tab.cifar}.}
% \vspace{-10pt}
\resizebox{1\linewidth}{!}{%
\centering
% \normalsize
\setlength{\tabcolsep}{8pt}
\begin{tabular}{l|c|ccc|c}
\toprule[1pt]
% \hline
\multicolumn{1}{c|}{Method} & Ref.      & Many           & Medium         & Few            & All            \\ \midrule[1pt]
CE++                    & -         & \textbf{81.76} & 54.85          & 10.82          & 48.76          \\
CB                          & CVPR19    & 75.94          & 50.00          & 18.27          & 50.28          \\
LDAM                        & NeurIPS19 & 74.33          & 51.11          & 19.87          & 50.34          \\
$\tau$ Norm                    & ICLR20    & 74.17          & 53.89          & 24.47          & 52.41          \\
RIDE                        & ICLR21    & 77.06          & 55.33          & 24.87          & 54.72          \\
LA                   & ICLR21    & 78.94          & 56.97          & 25.12          & 55.35          \\
MiSLAS                      & CVPR21    & 75.94          & 58.77          & 28.87          & 56.12          \\
TADE                        & ICCV21    & 81.26 & 57.74          & 19.53          & 55.73          \\
Prior-LT                    & NeurIPS21 & 79.17          & 58.14          & 26.60          & 56.22          \\
LTR-WD                      & CVPR22    & 77.26          & 56.39          & 22.53          & 54.32          \\
GCL                         & CVPR22    & 78.94          & 57.47          & 27.94          & 56.88          \\ \midrule[1pt]
Ours                        & -         & 77.94          & \textbf{59.23} & \textbf{30.77} & \textbf{57.24} \\
% \hline
\bottomrule[1pt]
\end{tabular}}
% \vspace{-15pt}
\label{Tab.result_new_baseline}
\end{table}
